Focus on What Matters: Enhancing Medical Vision-Language Models with Automatic Attention Alignment Tuning

Medical Large Vision-Language Models (Med-LVLMs) often exhibit suboptimal attention distribution on visual inputs, leading to hallucinated or inaccurate outputs. Existing mitigation methods primarily rely on inference-time interventions, which are limited in attention adaptation or require additional supervision. To address this, we propose A$^3$Tune, a novel fine-tuning framework for Automatic Attention Alignment Tuning. A$^3$Tune leverages zero-shot weak labels from SAM, refines them into prompt-aware labels using BioMedCLIP, and then selectively modifies visually-critical attention heads to improve alignment while minimizing interference. Additionally, we introduce a A$^3$MoE module, enabling adaptive parameter selection for attention tuning across diverse prompts and images. Extensive experiments on medical VQA and report generation benchmarks show that A$^3$Tune outperforms state-of-the-art baselines, achieving enhanced attention distributions and performance in Med-LVLMs.

==> ACL2025-latex/1_introduction.tex <==
\section{Introduction}

% Paragraph 1: \ul{The developments of Med-LVLMs and Problems in Med-LVLMs..}



\begin{figure*}[h!]
  \centering
  \includegraphics[width=0.95\linewidth]{ACL2025-latex/figures/Preliminary_Cases_v5.pdf}
  \vspace{-0.1in}
  \caption{(A) Examples of medical VQA and attention maps on medical images. In this example of Brain MRI from the SLAKE dataset, red box denotes the RoI of the brain tumor that LLaVA-Med should focus on. Red texts and green texts indicate wrong answers and correct answers, respectively. (B) Example of ground truth RoIs for different prompts on an Abdomen CT from SLAKE.}
  \vspace{-0.1in}
  \label{fig:preliminary}
\end{figure*}


% \ul{Issues in Med-LVLMs and an example to show the attention distribution bias.}
Medical Large Vision-Language Models (Med-LVLMs), represented by LLaVA-Med~\cite{li2024llava}, have shown significant progress in medical domains~\cite{chexagent-2024, thawkar2023xraygpt, moor2023med}, excelling in tasks like medical image interpretation and clinical decision-making.
Despite their potential, Med-LVLMs often produce inaccurate or hallucinated outputs that deviate from the provided visual medical information, as revealed by recent benchmarks~\cite{xia2024cares, gu2024medvh, chen2024detecting}. 

An example of medical visual question answering (VQA) extracted from the SLAKE~\cite{liu2021slake} dataset is shown in Figure~\ref{fig:preliminary}(A), where we visualize the average attention map on the image inputs during generating answers. We can observe that LLaVA-Med in Figure~\ref{fig:preliminary}(A.2) generates the hallucinated response ``\textit{Alzheimer's disease}'', neglecting the tumor region and over-focusing on irrelevant background areas, as shown in the corresponding attention map. This reveals a significant bias in attention distribution on visual inputs that limits the model’s effectiveness. Similar attention biases have been identified in general LVLMs~\cite{gong2024damro, woo2024don, liu2025paying}.


% Inherited from 
% \ul{Existing mitigation methods focusing on the attention side.}
Existing methods for general LVLMs primarily use \textbf{inference-time} interventions to address these issues. Contrastive decoding is commonly used to mitigate two key types of attention bias: (i) over-reliance on textual information~\cite{leng2024mitigating, favero2024multi, liu2025paying}, and (ii) excessive attention to irrelevant background visual tokens~\cite{woo2024don, gong2024damro} by introducing a contrastive adjustment to the decoding logits. However, this approach does not directly modify the attention distribution, meaning it cannot ensure the model attends to diagnostically critical regions.
ControlMLLM~\cite{wu2024controlmllm}, takes a different approach by directly modifying attention maps during inference, ensuring the model focuses on pre-annotated regions of interest (RoIs). However, as shown in Figure~\ref{fig:preliminary}(A.3), it still produces partially hallucinated content. Additionally, it requires additional tuning and ground truth RoIs during every inference process, making it impractical for real-world applications.

% This method aims to reduce attention issues such as (i) over-reliance on textual information~\cite{leng2024mitigating, favero2024multi, liu2025paying} (for example, PAI~\cite{liu2025paying} manually increases the attention score on visual inputs and detract the logits generated using text-only information, to decrease such attention bias)and (ii) excessive attention to irrelevant background visual tokens~\cite{woo2024don, gong2024damro}, for example, DAMRO~\cite{gong2024damro} tries to decrease the bias introduced by high attention on background visual tokens by minus the decoding logits generated using only top background tokens with high attention. 



% \ul{Introduce fine-tuning to mitigate such issues and the subsequent challenges.} 
To overcome the limitations of inference-time intervention, an ideal solution is to automatically adjust attention maps towards RoIs during fine-tuning for downstream medical tasks. This approach enables the model to place more attention on critical regions during inference, eliminating the need for additional labels or interventions.  However, implementing such a method poses several challenges:

\textbf{(1) Limited availability of medical segmentation labels.} As shown in Figure~\ref{fig:preliminary}(A.3), using segmentation labels (RoIs) as guidance, as done in ControlMLLM, can enhance the learning of accurate attention maps and answer correctness. However, such labels are often unavailable in medical datasets and real-world applications.

\textbf{(2) Trade-off between attention alignment and model stability.} Assuming that RoI labels are available, directly modifying the attention maps of all attention heads towards the labels without any strategy is still risky. This may lead to the over-alignment issue that potentially impacts the output stability and overall performance. Therefore, achieving the right balance between attention alignment and model stability is essential.
% thus creating a trade-off between attention alignment and performance. How to achieve a balance is essential.

\textbf{(3) Adapting attention to diverse prompts and images.} Even if attention alignment and model stability are balanced, the parameter-sharing strategy in fine-tuning remains a limitation for adaptive attention alignment. For example, as shown in Figure~\ref{fig:preliminary}(A) and (B), the optimal RoIs can vary significantly based on the input prompt and image, requiring dynamic alignment. While the computation of attention maps adjusts to input representations, the shared parameters in fine-tuning limit the model's ability to flexibly learn attention distribution across diverse inputs.


\begin{figure*}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{ACL2025-latex/figures/model_figure_v1.pdf}
  \vspace{-0.1in}
  \caption{The overview of \ours.}
  \label{fig:model_design}
  \vspace{-0.1in}
\end{figure*}

To address these challenges simultaneously, we propose \ours, a novel fine-tuning framework designed for \textbf{A}utomatic \textbf{A}ttention \textbf{A}lignment \textbf{Tuning}. As shown in Figure~\ref{fig:model_design}, \ours integrates a  set of cooperative strategies to ensure that attention in Med-LVLMs is well aligned, minimally disruptive, and highly adaptable across diverse medical tasks. Firstly, to overcome the lack of segmentation labels (Challenge 1), \ours utilizes zero-shot segmentation labels generated by SAM~\cite{roy2023sam} and further refines them into prompt-aware weak labels using BioMedCLIP~\cite{zhang2023biomedclip}. These weak labels serve as guidance for attention alignment, eliminating the need for manual annotations. 
However, weak labels alone are not sufficient — uncontrolled modifications on all attention heads can disrupt model stability (Challenge 2). To further balance attention alignment with model stability, \ours selectively modifies only the most ``visually-critical'' attention heads, minimizing the risk of over-alignment and instability. Furthermore, the parameter-sharing strategy in alignment tuning remains a limitation, as RoIs vary significantly based on the input prompt and image (Challenge 3). To address this, we incorporate a custom-designed \textbf{M}ixture-\textbf{o}f-\textbf{E}xperts \moe into \ours on attention modules, allowing the model to dynamically select parameters and adjust attention maps for different images and prompts.
% even with balanced attention alignment using weak labels,
% However, weak labels alone are not sufficient — uncontrolled attention modifications can disrupt model performance. 

% Our experiments across diverse benchmarks in medical VQA and report generation demonstrate the effectiveness of \ours in improving attention distribution on RoIs and overall performance.
In summary, this work makes the following contributions:
\begin{itemize}
    % \item We conduct an in-depth analysis of attention distribution on visual tokens and its critical role in the decision-making process of Med-LVLMs.
    % \item We reveal a significant attention distribution bias on visual inputs in Med-LVLMs that limits the model’s effectiveness.
    \item We propose \ours, a novel visual attention tuning approach that utilizes zero-shot weak labels to refine the visual focus of Med-LVLMs and enhance their performance.
    \item We develop a set of designs for cooperative attention alignment tuning: (i) weak label supervision, (ii) selective tuning of visually-critical attention heads, and (iii) a \moe module for adaptive attention adjustment.
    \item We conduct extensive experiments on five medical VQA and two report generation benchmarks against ten baselines, demonstrating that \ours outperforms state-of-the-art methods in both effectiveness and interpretability, improving visual grounding and overall model performance.
\end{itemize} 


% To overcome the drawbacks of the existing methods, an ideal way is to automatically direct the attention towards RoIs without relying on inference-time intervention and ground truth labels. To achieve this, we propose to add guidance on visual attention during fine-tuning for downstream tasks, enabling the model to automatically focus on RoIs during downstream inference without additional intervention. This forms the foundation of our proposed method, automatic xxx, \textbf{V}isual \textbf{A}ttention \textbf{T}uning (\ours) (here, think about a new name not just simply about visual atteniton tuning, including contributed designs). However, challenges exist to implement and achieve  such a tuning:

% To investigate this, we analyze LLaVA-Med as a representative Med-LVLM, focusing on its attention distribution on visual tokens. Our analysis reveals an attention bias: as shown in Figure~\ref{fig:preliminary}(a), LLaVA-Med often assigns low attention to diagnostically significant regions while over-focusing on background tokens. This suboptimal attention distribution likely contributes to visually ungrounded and inaccurate outputs.

% Our preliminary experiments confirm this hypothesis. By directly tuning attention distribution toward regions of interest (RoIs) at inference time using ControlMLLM~\cite{wu2024controlmllm}, LLaVA-Med can rectify ungrounded answers (Figure~\ref{fig:preliminary} (b)). With further experiments of inference time tuning on more data  in Section~\ref{sec:preliminary}, we find that there is a positive correlation between attention to RoIs and VQA performance, highlighting the importance of attention distribution on visual tokens.

% Paragraph 3: \ul{Research Gaps 01. Existing hallucination mitigation methods with a focus on visual token interactions.} Current methods have proposed solutions to visual-textual interaction biases in LVLMs by constructing negative logits within contrastive decoding frameworks. These methods aim to mitigate two prominent issues: (1) excessive dependence on textual inputs, leading to insufficient attention to visual data and subsequent hallucinations~\cite{leng2024mitigating, favero2024multi, liu2025paying}, and (2) biases within visual inputs, such as high attention on irrelevant background visual tokens~\cite{woo2024don, gong2024damro}. Despite these efforts, there remains a lack of detailed exploration into how attention is distributed across different visual regions and how this influences the LVLM's decision-making

% Paragraph 4: \ul{Research Gaps 02. Our observation: suboptimal attention distribution on visual tokens.} In our method design, we first analyze the attention distribution on different visual tokens and regions based on LLaVA-Med, a representative Med-LVLM. We identify a critical gap in how LLaVA-Med interact with visual tokens: Different with LVLMs such as LLaVA in general domain tasks,   LLaVA-Med often assign low attention to diagnostically significant regions in medical tasks. This suboptimal attention distribution and lack of targeted interaction on visual tokens undermines the reliability of medical LLaVA-Med.

% Paragraph 5: \ul{Preliminary experiment and our motivations.} This observation raises a critical question: Can redirecting attention to correct visual regions help mitigate hallucination issues? To investigate this, we conducted preliminary experiments using a visual prompt tuning method to guide attention towards critical regions during inference. The results show that Med-LVLMs can improve their responses when attention is explicitly focused on regions of interest. However, simply tuning attention distribution at inference time requires accurate segmentation labels, which are often unavailable in medical settings, and this approach incurs additional tuning costs during every inference process. These challenges and findings motivate the development of methods that refine visual attention during pre-training or fine-tuning, particularly when only weak or limited segmentation labels are available.





==> ACL2025-latex/trash.tex <==
\begin{table*}[t]
\centering
\caption{Results on medical VQA benchmarks. The best results are highlighted in \textbf{bold}, and the second-best results are \ul{underlined}. OmniVQA represents the dataset OmniMedVQA.}
\label{tab:main_exp_vqa}
\vspace{-0.1in}
\resizebox{1.8\columnwidth}{!}{
\begin{tabular}{p{3.3cm}|cc|cc|cc|c|c}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Slake}} & \multicolumn{2}{c|}{\textbf{VQA-RAD}} & \multicolumn{2}{c|}{\textbf{PathVQA}} & \multicolumn{1}{c|}{\textbf{IU-Xray}} & \multicolumn{1}{c}{\textbf{OmniVQA}} \\
\cline{2-9}
 & \textbf{Open} & \textbf{Closed} & \textbf{Open} & \textbf{Closed} & \textbf{Open} & \textbf{Closed} & \textbf{Closed} & \textbf{Closed} \\
\midrule

\rowcolor{gray!15} LLaVA-Med & 41.28 & 57.75 & 32.48 & 68.90 & 10.34 & 52.49 & 72.83 & 31.79 \\
+ Greedy & 42.81 & 60.00 & \ul{38.61} & \ul{69.29} & 11.35 & 52.34 & 75.00 & 31.11  \\
+ Beam search & 42.31 & 61.69 & 34.90 & 66.54 & 9.86 & 53.79 & 73.59 & 30.89  \\
+ Nucleus sampling & 41.06 & 61.41 & 32.64 & 68.11 & 9.93 & 53.17 & 73.09 & 30.96  \\
+ VCD & 39.76 & 59.44 & 33.93 & 66.54 & 11.17 & 53.52 & 74.36 & 32.89 \\
+ DoLa & 42.37 & 59.72 & \textbf{38.78} & 68.50 & 11.38 & 52.55 & 74.87 & 31.04 \\
+ OPERA & 40.44 & 60.00 & 35.54 & 68.50 & 9.77 & 53.17 & 75.00 & 31.72 \\
+ AVISC & 41.46 & 59.72 & 35.43 & 64.17 & 11.03 & 52.20 & 73.85 & 32.48 \\
+ M3ID & 38.85 & 60.28 & 35.31 & 62.60 & 9.80 & 52.93 & 72.32 & 31.11 \\
+ DAMRO & 41.33 & 59.72 & 32.73 & 66.54 & 10.80 & 51.84 & 72.19 & 31.45  \\
+ PAI & 43.18 & 60.28 & 36.77 & 68.50 & 11.09 & 52.46 &  74.87 & 32.13 \\

\midrule
\rowcolor{gray!15} LLaVA-Med + LoRA & 80.65 & 82.82 & 33.37 & 66.54 & 31.92 & 90.95 & 83.29 & 90.65 \\
+ Greedy  & 81.12  & 85.07 & 31.88 & 68.50 & 33.90 & 91.86 & 83.93 & 90.73  \\
+ Beam search & 81.32 & \textbf{86.76} & 32.55 & 68.90 & 33.60 & \ul{91.92} & 84.06 & 90.58\\
+ Nucleus sampling & 80.18 & 85.35 & 31.34 & 68.50 & 30.14 & 90.92 & 83.41&90.05 \\
+ VCD & 79.58 & 84.23 & 32.96 & 67.72 & 30.20 & 90.86 & 83.93&90.73\\
+ DoLa & 81.84 & \ul{86.48} & 31.94 & 68.50 & \ul{34.00} & 91.86 & 84.06 &90.69 \\
+ OPERA & 81.25 & \ul{86.48} & 33.18 & 68.90 & 33.64 & 91.80 & 84.06 &90.42 \\
+ AVISC & 80.15 & 85.63 & 33.66 & \ul{69.29} & 32.37 & 90.62 & 84.06 & 90.54 \\
+ M3ID & 79.83 & 84.79 & 31.40 & 68.90 & 32.47 & 91.15 & \ul{84.95} & 90.73\\
+ DAMRO & \ul{82.19} & 83.66 \\
+ PAI & 81.02 & \textbf{86.76} & 32.14 & 68.11 & 33.46 & 91.77 & 84.31 & \ul{90.95}\\
\midrule
LLaVA-Med + \ours & \textbf{82.36} & \textbf{86.76} & 36.97 & \textbf{70.87} & \textbf{34.61} & \textbf{92.19} & \textbf{85.97} & \textbf{91.98}\\
\bottomrule
\end{tabular}}
% \vspace{-0.1in}
\end{table*}


\begin{table*}[t]
\centering
\caption{Results on report generation benchmarks based on LLaVA-Med fine-tuned with LoRA.}
\label{tab:main_exp_report_02}
\vspace{-0.1in}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{p{1.3cm}|p{1.8cm}|ccccccccccc|c}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Metric}} & \multicolumn{12}{c}{\textbf{Method}}\\
\cline{3-14}
& & \makecell{LLaVA-Med \\ + LoRA} 
& \makecell{+ \\ Greedy} 
& \makecell{+ \\ Beam} 
& \makecell{+ \\ Nucleus} 
& \makecell{+ \\ VCD} 
& \makecell{+ \\ DoLa} 
& \makecell{+ \\ OPERA} 
& \makecell{+ \\ AVISC} 
& \makecell{+ \\ M3ID} 
& \makecell{+ \\ DAMRO} 
& \makecell{+ \\ PAI} 
& \makecell{LLaVA-Med \\ + \ours} \\
% & \makecell{+ \\ \ours} \\
\midrule
\multirow{7}{*}{\textbf{IU-Xray}} & \textbf{BLEU} & 7.70 & 8.86 & \ul{9.34} & 7.80 & 8.83 & 8.93 & 8.27 & 8.52 & 8.63 & 7.29 & 8.87 & \textbf{11.05} \\
& \textbf{ROUGE-L}  & 26.15 & 27.09 & 27.56 & 26.72 & 27.36 & 26.94 & 27.14 & 26.97 & \ul{27.79} & 25.61 & 26.74 & \textbf{30.00} \\
& \textbf{METEOR}  & 29.50 & 26.01 & 26.44 & 30.33 & \ul{31.77} & 25.74 & 29.66 & 31.14 & 31.65 & 30.03 & 25.99 & \textbf{34.26} \\
& \textbf{BERTScore}  & 88.36 & 88.50 & \ul{88.52} & 88.28 & 88.30 & 88.42 & 88.41 & 88.47 & \ul{88.52} &88.14 & 88.39 & \textbf{89.05} \\
& \textbf{CheXbert}  & 53.81 & 52.55 & 52.88 & 52.73 & 51.86 & 52.27 & \ul{56.26} & 53.33 & 54.45 & 51.50 & 52.45 & \textbf{57.19} \\
& \textbf{RadGraph}  & 20.44 & 20.76 & 21.29 & 20.85 & 22.02 & 20.63 & 21.87 & \ul{22.27} & 22.22 & 20.75 & 20.48 & \textbf{24.24} \\
& \textbf{RaTEScore}  & 58.37 & 58.24 & 58.77 & 57.84 & 58.93 & 58.10 & 58.73 & 59.21 & \ul{59.37} &59.19 & 57.81 & \textbf{63.03} \\
\midrule
\multirow{7}{*}{\makecell{\textbf{MIMIC-}\\\textbf{CXR}}} & \textbf{BLEU} & 3.28 & 4.07 & 3.39 & 3.29 & 3.53 & 3.99 & 3.14 & 3.34 & 3.62 & 3.37 & \ul{4.32} & \textbf{4.56} \\
& \textbf{ROUGE-L} & 16.54 & \ul{18.75} & 17.25 & 16.14 & 16.58 & 18.62 & 15.52 & 16.79 & 16.67 & 15.75 & 18.64 & \textbf{19.03} \\
& \textbf{METEOR} & 17.90 & 18.81 & 17.36 & 17.98 & 18.68 & 18.68 & 14.70 & 18.29 & 18.22 & 17.03 & \ul{19.78} & \textbf{20.23} \\
& \textbf{BERTScore} & 85.57 & \ul{86.14} & 85.78 & 85.42 & 85.57 & \ul{86.14} & 84.75 & 85.59 & 85.58 &85.27 & 86.10 & \textbf{86.17} \\
& \textbf{CheXbert} & 22.14 & 24.24 & 23.05 & 21.76 & 23.38 & \ul{25.14} & 20.07 & 22.74 & 22.95 & 22.76 & \textbf{25.78} & 24.93 \\
& \textbf{RadGraph} & 9.43 & 10.73 & 9.78 & 9.20 & 9.93 & 10.75 & 7.74 & 9.52 & 9.93 & 9.40 & \ul{11.17} & \textbf{11.55} \\
& \textbf{RaTEScore} & 40.00 & \ul{41.06} & 38.59 & 39.26 & 40.95 & 40.73 & 35.72 & 40.08 & 39.87 & 39.62 & 41.03 & \textbf{42.73} \\
\bottomrule
\end{tabular}}
% \vspace{-0.1in}
\end{table*}
